Differentiable graph-structured models for inverse design of lattice materials

Architected materials possessing physico-chemical properties adaptable to disparate environmental conditions embody a disruptive new domain of materials science. Fueled by advances in digital design and fabrication, materials shaped into lattice topologies enable a degree of property customization not afforded to bulk materials. A promising venue for inspiration toward their design is in the irregular micro-architectures of nature. However, the immense design variability unlocked by such irregularity is challenging to probe analytically. Here, we propose a new computational approach using graph-based representation for regular and irregular lattice materials. Our method uses differentiable message passing algorithms to calculate mechanical properties, therefore allowing automatic differentiation with surrogate derivatives to adjust both geometric structure and local attributes of individual lattice elements to achieve inversely designed materials with desired properties. We further introduce a graph neural network surrogate model for structural analysis at scale. The methodology is generalizable to any system representable as heterogeneous graphs.

==> content/figures.tex <==
\showJournal{\begin{figure}[tb!]
    \centering    \includegraphics[width=112mm]{figures/Figure1.pdf}
	\caption{
	Schematic illustration of the proposed framework. A lattice material is represented as a graph $\mathcal{L}$ (left) which contains vector attributes both on the nodes (e.g. position) and edges (e.g. Young's modulus and beam cross-sectional area).
	A differential forward model $F$ takes the graph as input and predicts material properties.
	Comparing these predictions with desired properties, automatic differentiation is used to change the material (e.g., move nodes and remove or add beams) to better satisfy those properties.
	This process is repeated iteratively until a material with the desired properties is found.
	}\vspace{-5.8mm}	
	\label{fig:intro}
\end{figure}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=172mm]{figures/Figure2.pdf}
	\caption{
	Comparison of analytical values (\cref{tab:rels}) and values obtained using our finite element method.
    We show the effective elastic modulus (left) and Poisson's ratio (right) for different tilings (square, equilateral triangle, honeycomb and reentrant honeycomb) and relative densities.
    To change the relative density, we repeated numerical experiments for lattices with different number of cells and beam cross-areas.
	}\vspace{-2mm}	
	\label{fig:analytical}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=172mm]{figures/Figure3.pdf}
	\caption{
	Illustration of the message passing steps. For clarity, we only show the operations on one edge, although in practice, these operations are performed on all edges in parallel. 
	(1) Node features $\pmb r_i$ are propagated along connecting edges.
	(2) On the edges, propagated node features as well as edge features are combined via a function $\phi_0$ to create new edge features. $\phi_0$ can take any shape (e.g., a neural network).
	(3) Edge features are reduced using a function $\phi_1$ that satisfies permutation invariance (i.e., the order of arguments does not matter) and is applicable to a varying number of arguments.
	(4) The node features are updated using the reduced edge features using a function $\phi_2$ (which, again, can take any shape).
	}\vspace{-4mm}	
	\label{fig:MP}
\end{figure*}

\begin{figure}[t!]
    \centering
    \includegraphics[width=112mm]{figures/Figure4.pdf}
	\caption{
	Illustration of message passing finite element. Using message passing on the graph representation of the lattice, first the stiffness matrix of each beam is computed (locally on each edge of the graph), from which the global stiffness matrix $G$ is then constructed (by pooling from all edges).
	}\vspace{-4mm}	
	\label{fig:MPFE}
\end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=172mm]{figures/Figure5.pdf}
	\caption{
	Inverse designing lattices to have desired mechanical properties. 
	Lattices without load are shown in light gray and with load in black.
	Top nodes (red) are forced, while bottom nodes (gray) are constrained to not move. In the middle plots, target values of properties are shown as dashed lines. 
    \textbf{(A)} Inverse designing a square lattice to have a higher effective elastic modulus while keeping the relative density constant. Deformations are magnified by a factor of $10$. 
    \textbf{(B)} Inverse designing a triangle lattice to have a negative Poisson's ratio while keeping the relative density constant. Deformations are not magnified.
	}\vspace{-4mm}	
	\label{fig:invDesign_Stiffness}
 \label{fig:invDesign_Poisson}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=172mm]{figures/Figure6.pdf}
	\caption{
	Inverse designing a lattice to yield certain deformation responses to loads. Colors and line styles as in \cref{fig:invDesign_Stiffness}. Nodes with target behaviour are shown as colored squares.
    \textbf{(A)} Inverse design of a grabbing tool. 
    Progress towards the target for all four nodes is shown in the middle plot, colored like the corresponding nodes (left and right, colored squares).
    In the lattice illustrations (left and right), target deformations are indicated by crosses. A lever-like structure that emerged during inverse design is highlighted in gold.
    Deformations are magnified by a factor of $4$. See also Video S1.
    \textbf{(B)} Inverse designing the response to two different load scenarios.
    As can be seen in the middle figure, if we only train on load scenario 1, the target behaviour for load scenario 2 is not reached.
    However, training on both scenarios will lead to a solution that satisfies both target behaviours.
    Deformations are magnified by a factor of $5$. See also \cref{fig:invDesign_FlatSI} and Video S2. \textbf{(C)} Inverse designing a large honeycomb lattice to have zero Poisson's ratio. Initially, loading the lattice leads to a bulging outwards. With our framework, a design is found that leads to no bulging, featuring local tiling motives resembling tilted reentrant honeycombs and triangles. See also \cref{fig:LargeAuxMagnified} and Video S3.
	}\vspace{-4mm}	
	\label{fig:invDesign_Grab}
    \label{fig:invDesign_Flat}
    \label{fig:Large}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=172mm]{figures/Figure7.pdf}
	\caption{Experiments using graph neural networks as the forward model. \textbf{(A)} Model prediction vs. ground truth for the EdgeConv model. \textbf{(B)}
	Inverse design using a GNN as the forward model $F$. 
	A triangle lattice is adjusted to feature a reduced effective elastic modulus while its relative density has to be unchanged.
	Target values for the elastic modulus and relative density are shown as dashed lines.
	The predicted value by the GNN $F(\mathcal{L})$ is shown in blue (straight line), while the exact value obtained using finite element is shown in red (dashed dotted line).
	Colors and line styles as in \cref{fig:invDesign_Stiffness}.
	Deformations are magnified by a factor of $2$. See also \cref{fig:invDesignTrain}.
	}\vspace{-4mm}	
	\label{fig:invDesign_GNN}
 \label{fig:prediction}
\end{figure*}

\begin{figure}[t!]
    \centering
    \includegraphics[width=112mm]{figures/Figure8.pdf}
	\caption{
	Experimental setup for determining both the effective elastic modulus and the Poisson's ratio of a lattice material along the loading direction. The material -- here a lattice with honeycomb tiling -- is placed between two plates. By pressing the top plate downwards while keeping the bottom plate unmoved, the material gets compressed. With this approach, stress-strain as well as strain-strain curves are derived, from which the above-mentioned material properties are calculated.
	}\vspace{-4mm}	
	\label{fig:exp}
\end{figure}}
